Source Tracking for Sco X-1

Sco X-1, the brightest low mass X-ray binary, is likely to be a source for gravitational wave emission. In one mechanism, emission of a gravitational wave arrests the increase in spin frequency due to the accretion torque in a low mass X-ray binary. Since the gravitational waveform is unknown, a detection method assuming no apriori knowledge of the signal is preferable. In this paper, we propose to search for a gravitational wave from Sco X-1 using a {{\it source tracking}} method based on a coherent network analysis. In the method, we combine data from several interferometric gravitational wave detectors taking into account of the direction to Sco X-1, and reconstruct two polarization waveforms at the location of Sco X-1 in the sky as Sco X-1 is moving. The source tracking method opens up the possibility of searching for a wide variety of signals. We perform Monte Carlo simulations and show results for bursts, modeled, short duration periodic sources using a simple excess power and a matched filter method on the reconstructed signals.

==> Makefile <==
LATEX=latex
DVIPS=dvips
BIBTEX=bibtex
TEXFILE=scox1
DVIPDF=dvipdfmx

build:
	${LATEX} ${TEXFILE}.tex
	${BIBTEX} ${TEXFILE}
	${LATEX} ${TEXFILE}.tex
	${LATEX} ${TEXFILE}.tex
	${DVIPDF} ${TEXFILE}.dvi
view:
#	open -a Adobe\ Reader ${TEXFILE}.pdf &
	open -a preview ${TEXFILE}.pdf &
print:
	lpr -Plp ${TEXFILE}.ps
#miniprint:
#	psnup -2 ${TEXFILE}.ps | psprint -flip -
pdf:
	ps2pdf ${TEXFILE}.ps
edit	:
	mate $(TEXFILE).tex
clean:
	rm -f ${TEXFILE}.log ${TEXFILE}.aux ${TEXFILE}.log ${TEXFILE}.dvi ${TEXFILE}.bbl ${TEXFILE}.blg ${TEXFILE}.toc *~

